A web-based IDE for IDP

IDP is a knowledge base system based on first order logic. It is finding its way to a larger public but is still facing practical challenges. Adoption of new languages requires a newcomer-friendly way for users to interact with it. Both an online presence to try to convince potential users to download the system and offline availability to develop larger applications are essential. We developed an IDE which can serve both purposes through the use of web technology. It enables us to provide the user with a modern IDE with relatively little effort.

==> idp-latex/idp-latex.tex <==
%IMPORTANT: ONLY INCLUDE AS \input{idp-latex/idp-latex}
\usepackage{import}

\subimport{idp-latex/}{includes-no-theorems}
\subimport{idp-latex/}{common-citations}
\subimport{idp-latex/}{theorems}


==> idp-latex/theorems.tex <==
\usepackage{amsthm}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem*{lem*}{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{lemma}[thm]{Lemma}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}

\newtheorem{nota}[thm]{Notation}
\newtheorem*{nota*}{Notation}


\newtheoremstyle{example_basic} 
{\topsep} %ABOVESPACE
{\topsep} %BELOWSPACE 
{\normalfont}% Body font 
{0pt}% Indent amount (empty = no indent, \parindent = para indent) 
{\bfseries}% Thm head font 
{.}% Punctuation after thm head 
{5pt plus 1pt minus 1pt}% Space after thm head (\newline = linebreak) 
{}% Thm head spec

\newtheoremstyle{example_contd}
{\topsep} %ABOVESPACE
{\topsep} %BELOWSPACE 
{\normalfont}% Body font 
{0pt}% Indent amount (empty = no indent, \parindent = para indent) 
{\bfseries}% Thm head font 
{.}% Punctuation after thm head 
{5pt plus 1pt minus 1pt}% Space after thm head (\newline = linebreak) 
{\thmname{#1} \thmnumber{ #2}\thmnote{#3} (continued)}% Thm head spec 

\theoremstyle{example_basic} 
\newtheorem{ex}[thm]{Example}
\newtheorem{example}[thm]{Example}
\newtheorem{remark}[thm]{Remark}

\newtheorem{ex*}{Example}
\theoremstyle{example_contd} 
\newtheorem*{ex_continued}{Example}

\theoremstyle{plain}



